PANDA : Perceptually Aware Neural Detection of Anomalies

Semi-supervised methods of anomaly detection have seen substantial advancement in recent years. Of particular interest are applications of such methods to diverse, real-world anomaly detection problems where anomalous variations can vary from the visually obvious to the very subtle. In this work, we propose a novel fine-grained VAE-GAN architecture trained in a semi-supervised manner in order to detect both visually distinct and subtle anomalies. With the use of a residually connected dual-feature extractor, a fine-grained discriminator and a perceptual loss function, we are able to detect subtle, low inter-class (anomaly vs. normal) variant anomalies with greater detection capability and smaller margins of deviation in AUC value during inference compared to prior work whilst also remaining time-efficient during inference. We achieve state of-the-art anomaly detection results when compared extensively with prior semi-supervised approaches across a multitude of anomaly detection benchmark tasks including trivial leave-one out tasks (CIFAR-10 - AUPRCavg: 0.91; MNIST - AUPRCavg: 0.90) in addition to challenging real-world anomaly detection tasks (plant leaf disease - AUC: 0.776; threat item X-ray - AUC: 0.51), video frame-level anomaly detection (UCSDPed1 - AUC: 0.95) and high frequency texture with object anomalous defect detection (MVTEC - AUCavg: 0.83).

==> tables/table_mvtec.tex <==
\begin{table*}[h!]
\caption{AUPRC results across MVTEC \cite{Bergmann2019MVTEC} dataset.}
\label{tab:mvtec}

\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\bf Model} & \multicolumn{15}{c|}{\textbf{Classes}} \\ \cline{2-16}
& \textbf{Bottle} & \textbf{Cable} & \textbf{Capsule} & \textbf{Carpet} & \textbf{Grid} & \textbf{Hazelnut} & \textbf{Leather} & \textbf{Metal Nut} & \textbf{Pill} & \textbf{Screw} & \textbf{Tile}  & \textbf{Toothbrush} & \textbf{Transistor} & \textbf{Wood}  & \textbf{Zipper} \\ \hline \hline
\rowcolor{gray!15}
AnoGAN \cite{Schlegl2017}        & 0.8             & 0.477          & 0.442            & 0.337           & 0.871         & 0.259             & 0.451            & 0.284              & 0.711         & 1              & 0.401          & 0.439               & 0.692               & 0.567          & 0.715           \\ 
GANomaly\cite{Akcay2018}      & 0.794           & \textbf{0.711} & 0.721            & 0.821           & 0.743         & 0.874             & 0.808            & 0.694              & 0.671         & 1              & 0.72           & 0.7                 & 0.808               & 0.92           & 0.744           \\ 
\rowcolor{gray!15}
Skip-GANomaly\cite{Akcay2019}  & 0.937           & 0.674          & 0.718            & 0.795           & 0.657         & 0.906             & 0.908            & 0.79               & 0.758         & 1              & 0.85           & 0.689               & 0.814               & 0.919          & 0.663           \\ 

DA-GAN \cite{Tang2020}        & \textbf{0.983}  & 0.665          & 0.687            & 0.903           & 0.867         & \textbf{1}        & \textbf{0.944}   & \textbf{0.815}     & 0.768         & 1              & 0.961          & \textbf{0.95}                & 0.794               & \textbf{0.979} & \textbf{0.781}  \\ 
\rowcolor{gray!15}
U-Net \cite{Ronneberger2015}        & 0.863           & 0.636          & 0.673            & 0.774           & 0.857         & 0.996             & 0.87             & 0.676              & 0.78          & 1              & \textbf{0.964} & 0.811               & 0.674               & 0.958          & 0.75            \\
\rowcolor{blue!8}
\textbf{PANDA-GAN}     & 0.826           & 0.68           & \textbf{0.98}    & \textbf{0.95}   & \textbf{0.95} & 0.922             & 0.75             & 0.79               & \textbf{0.95} & \textbf{1}     & 0.85           & 0.66                & \textbf{0.9}        & 0.68           & 0.62            \\ \hline
\end{tabular}
}


\end{table*}
